Study of accelerator neutrino interactions in a liquid argon TPC

We study the potentialities of a 50 liter liquid argon TPC prototype operated at the CERN WANF neutrino beam. We concentrate on the selection and reconstruction of quasi-elastic events and measure the cross section for this reaction.

==> Theory/FeynDiag/DISscattering.tex <==
\fmfleft{N,nu}\fmflabel{$\nu(k)$}{nu}\fmflabel{$N(p_N)$}{N}
\fmfright{d0,o1,o2,d1,o3,d2,d3,d4,d5,d6,mu}\fmflabel{$q_2$}{o3}\fmflabel{$\mu(k^{\prime})$}{mu}
\fmf{fermion,tension=1.5}{nu,vnu}
\fmf{fermion}{vnu,mu}
\fmf{fermion,tension=3}{N,vp}
\fmf{fermion,tension=1,l.side=right}{vp,vq}
\fmf{fermion}{vq,o3}
\fmf{fermion}{vp,o1}
\fmf{fermion}{vp,o2}
\fmf{dashes_arrow,tension=1.5,l.side=left}{vnu,vq}
\fmfdot{vnu,vq}
\fmfblob{.15w}{vp}
\fmf{phantom,tension=0,label=$q_1(\xi p_N)$,l.side=left}{vp,vq}
\fmf{phantom,tension=0,label=$W^+(q)$,l.side=right}{vnu,vq}
\fmffreeze
\fmfi{plain}{vpath(__N,__vp) shifted (thick*(0,2))}
\fmfi{plain,l.side=right}{vpath(__N,__vp) shifted (thick*(1,-2))}
\fmfv{label=$U_{q_1 q_2}$,l.angle=23}{vq}
\fmf{dots,right,label=$X(p_X)$}{d0,d2}


==> Theory/FeynDiag/QECscattering.tex <==
\fmfstraight
\fmfleft{q1,q2,qd,d1,d2,d3,d4,d5,d6,d7,d8,d9,d10,nu}
\fmflabel{$N$}{q2}\fmflabel{$\nu$}{nu}
\fmfright{q1o,q2o,qc,d1o,d2o,d3o,d4o,d5o,d6o,d7o,d8,d9,d10o,mu}
\fmflabel{$B_c$}{q2o}\fmflabel{$\mu$}{mu}
\fmfcurved
\fmf{fermion}{nu,vl,mu}
\fmf{dashes,label=$W^{\pm}$}{vl,vq3}
\fmf{fermion,label=$d$,l.side=left}{qd,vq3}
\fmf{fermion,label=$c$,l.side=left}{vq3,qc}
\fmf{phantom,tension=5}{q1,anker,q1o}
\fmffreeze
\fmf{fermion}{q2,vq2,q2o}
\fmf{phantom,tension=5}{vq2,vq3}
\fmffreeze
\fmf{fermion}{q1,vq1,q1o}
\fmf{phantom,tension=5}{vq1,vq2}
\fmfdot{vl}
\fmfblob{.2w}{vq2}


==> Theory/FeynDiag/VertexGraph.tex <==
  \fmfleft{f1} \fmflabel{$f$}{f1}
  \fmfright{V,f2} \fmflabel{$V$}{V}\fmflabel{$f^{\prime}$}{f2}
  \fmfdot{Vff} \fmflabel{$g$}{Vff}
  \fmf{plain}{f1,Vff,f2}  
  \fmf{dashes}{Vff,V}


==> Theory/FeynDiag/ccprocess.tex <==
 \fmfleft{f2,f1} \fmflabel{$f_1$}{f1}\fmflabel{$f_2$}{f2}
 \fmfright{f2p,f1p} \fmflabel{$f_1^{\prime}$}{f1p}\fmflabel{$f_2^{\prime}$}{f2p}
 \fmfdot{Vf1,Vf2} \fmflabel{(1)}{Vf1}\fmflabel{(2)}{Vf2} 
 \fmf{plain}{f1,Vf1,f1p}
 \fmf{plain}{f2,Vf2,f2p}    
 \fmf{dashes,label=$W^{\pm}$,l.side=left}{Vf1,Vf2} 


==> Theory/FeynDiag/firstOrder.tex <==
\begin{tabular}{ccccc}
\fmfframe(5,10)(5,10){
\begin{fmfgraph*}(80,80)
  \fmfleft{d1,f2,d2,f1,lab} \fmflabel{$f_1$}{f1}\fmflabel{$f_2$}{f2}\fmflabel{(a)}{lab}
  \fmfright{dd1,f2p,dd2,f1p,dd3} \fmflabel{$f_1^{\prime}$}{f1p}\fmflabel{$f_2^{\prime}$}{f2p}
  \fmfdot{Vf1,Vf2} \fmflabel{$g$}{Vf1}\fmflabel{$g$}{Vf2} 
  \fmf{plain}{f1,Vf1,f1p}
  \fmf{plain}{f2,Vf2,f2p}    
  \fmf{dashes,label=$V$,l.side=left}{Vf1,Vf2} 
\end{fmfgraph*}
} &&
\fmfframe(5,10)(5,10){
\begin{fmfgraph*}(80,80)
  \fmfleft{d1,f2,d2,f1,lab} \fmflabel{$f_1$}{f1}\fmflabel{$f_2$}{f2}\fmflabel{(b)}{lab}
  \fmfright{dd1,f2p,dd2,f1p,dd3} \fmflabel{$f_1^{\prime}$}{f1p}\fmflabel{$f_2^{\prime}$}{f2p}
  \fmfdot{Vf1,Vf2} \fmflabel{$g$}{Vf1}\fmflabel{$g$}{Vf2} 
  \fmf{plain}{f1,Vf1,f2}
  \fmf{plain}{f1p,Vf2,f2p}    
  \fmf{dashes,label=$V$,l.side=left}{Vf1,Vf2} 
\end{fmfgraph*}
} &&
\fmfframe(5,10)(5,10){
\begin{fmfgraph*}(80,80)
  \fmfleft{d1,f2,d2,f1,lab} \fmflabel{$f_1$}{f1}\fmflabel{$f_2$}{f2}\fmflabel{(c)}{lab} 
  \fmfright{dd1,V2,dd2,V1,dd3} \fmflabel{$V$}{V1}\fmflabel{$V$}{V2}
  \fmfdot{Vf1,Vf2} \fmflabel{$g$}{Vf1}\fmflabel{$g$}{Vf2} 
  \fmf{plain}{f1,Vf1}
  \fmf{plain}{f2,Vf2}	  
  \fmf{plain,label=$f$,l.side=left}{Vf1,Vf2} 
  \fmf{dashes}{Vf1,V1} 
  \fmf{dashes}{Vf2,V2}
\end{fmfgraph*}
} \\
\end{tabular}


==> Theory/FeynDiag/nuNscattering.tex <==
\begin{tabular}{ccc}
\fmfframe(5,10)(5,10){
\begin{fmfgraph*}(160,140)
  \fmfleft{N,nu} \fmflabel{$\nu$}{nu}\fmflabel{$N$}{N}
  \fmfstraight
  \fmfright{x1,x2,x3,x4,d1,d2,d3,d4,d5,mu}\fmflabel{$X$}{x3}\fmflabel{$\mu$}{mu}
  \fmfcurved
  \fmflabel{$p_X$}{x2}
  \fmfdot{VnuMu}
  \fmfblob{.12w}{VNX}
  \fmf{fermion,label=$k$,l.side=left}{nu,VnuMu}
  \fmf{fermion,label=$k^{\prime}$,l.side=left}{VnuMu,mu}
  \fmf{fermion,label=$p_N$,l.side=right}{N,VNX}
  \fmf{fermion}{VNX,x2}
  \fmf{dashes,label=$W^{\pm}$,l.side=left,tension=.5}{VNX,VnuMu}
  \fmf{phantom,label=$q$,l.side=right,tension=0}{VNX,VnuMu}
  \fmffreeze
  \fmf{fermion,label=$p_h$,l.side=right}{VNX,x1}
  \fmf{fermion}{VNX,x3}
  \fmf{fermion}{VNX,x4}
\end{fmfgraph*}
} & &
\fmfframe(5,10)(5,10){
\begin{fmfgraph*}(160,160)
 \fmfcurved
 \fmfsurroundn{v}{40}%\fmfdotn{v}{40}
 \fmflabel{$\mu$}{v4}
 \fmflabel{$\nu$}{v21} 
 \fmflabel{$X$}{v38}
 \fmf{phantom}{v21,N,v1}
 \fmfdot{N}\fmflabel{$N$}{N}
 \fmf{fermion,label=$E$,l.side=left,tension=0}{v21,N}
 \fmf{dashes,tension=0}{N,v1}
 \fmf{fermion,label=$E^{\prime}$,l.side=left,tension=0}{N,v4}
 \fmf{fermion,tension=0}{N,v36}
 \fmf{fermion,tension=0}{N,v37}
 \fmf{fermion,tension=0}{N,v38}
 \fmf{fermion,tension=0}{N,v39}
 \fmffreeze
 \fmf{phantom}{N,du,au,v11}
 \fmf{phantom}{N,dd,ad,v31} 
 \fmf{phantom}{N,d1,a1,v4} 
 \fmf{phantom}{N,d1,a1,v4}
 \fmf{phantom}{N,d2,a2,v1}
 \fmffreeze
% \fmf{plain,left=0.1}{a1,a2}
 \fmf{phantom,left,tag=1}{au,ad}
 \fmfipath{p[]}
 \fmfiset{p1}{vpath1(__au,__ad)}
 \fmfi{plain,label=$\theta$,l.side=left}{subpath (7length(p1)/20,length(p1)/2) of p1}
 \end{fmfgraph*}
} \\
\\
$(a)$ && $(b)$
\end{tabular}


==> Theory/Tables/QECpredictionSummary.tex <==
\begin{tabular}{|l||>{$}  c  <{$}|>{$}  c  <{$}||>{$}  c  <{$}|>{$}  c  <{$}||>{$}  c  <{$}|>{$}  c  <{$}|}
\hline
 Process & \multicolumn{2}{c||}{$\nu_{\mu}n \rightarrow \mu\lambdac$}&\multicolumn{2}{c||}{$\nu_{\mu}n \rightarrow \mu\sigmacp$}& \multicolumn{2}{c|}{$\nu_{\mu}p \rightarrow \mu\sigmacpp$}\\ \cline{2-7}
$\sigma$ in $\unit[10^{-40}]{cm^2}$&\sigma&\nicefrac{\sigma}{\sigma_{cc}}&\sigma&\nicefrac{\sigma}{\sigma_{cc}}&\sigma&\nicefrac{\sigma}{\sigma_{cc}}\\\hline
Finjord, Ranvndal \cite{Finjord:1975fz} & 1.2 & \unit[0.18]{\%}  & 0.06  & \unit[0.009]{\%}  & 0.12  & \unit[0.018]{\%}\\ \hline
Shrock, Lee \cite{Shrock:1975uk,Shrock:1976Err}        & 23.0& \unit[3.4]{\%}  & 5.0  & \unit[0.74]{\%}  & 9.0  & \unit[1.3]{\%} \\ \hline
Avilez et al \cite{Avilez:1976bb,Avilez:1976qi,Avilez:1978rt}& 41.0 & \unit[6.1]{\%} & - & - & 8.4&\unit[1.3]{\%}\\ \hline
Amer et al \cite{Amer:1978ya}     & 3.2  & \unit[0.48]{\%}  & 0.6 & \unit[0.089]{\%} & 1.1 &\unit[0.17]{\%}\\ \hline
Kovalenko \cite{Kovalenko:1990zi}  & 5.0  & \unit[0.74]{\%}  & 1.5 & \unit[0.22]{\%} & 3.0  & \unit[0.45]{\%}\\ \hline
\end{tabular}


==> Theory/nNScatt.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Neutrino-Nucleon Scattering}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{sec:nNScatt}
As neutrinos are structureless and comparatively easy to produce in accelerators, they make an exceptional probe of hadronic matter. Investigating neutrino collisions in fixed target experiments is an excellent means for retrieving information about the structure of protons and neutrons. In order to provide a basis for further discussions of such scattering processes, some definitions have to be introduced. All the relevant expressions are given for charged current interactions, since this is what this thesis is concerned with. Also, since referring to the NOMAD experiment, the neutrino is always assumed to be a $\nu_{\mu}$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Kinematic Definitions}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{section:KinematicDefinitions}
Figure \ref{feyn:nuNscattering}(a) shows the Feynman diagram for neutrino-nucleon scattering:
\begin{equation}
\nu_{\mu} + N \rightarrow \mu^- + X
\label{eqn:nuNscattering}
\end{equation}
where $X$ denotes a not yet specified hadronic final state. The variables $k$ and $p_N$ denote the 4-momenta of the particles in the initial state, the neutrino and the nucleon. The 4-momentum of the final state muon is $k^{\prime}$. The hadronic final state is somewhat more complex as it may consist of several particles. Considered as a whole, it is assigned with the 4-momentum $p_X$ which is a sum of all the individual hadron 4-momenta $p_h$. The W-boson emitted by the neutrino carries the four-momentum $q$ which will be called 4-momentum transfer from here on.  

\begin{figure}[!htpb]
\begin{center}
\input{./Theory/FeynDiag/nuNscattering.tex}
\caption[Charged current neutrino-nucleon scattering]{Diagram for the reaction $\nu + N \rightarrow \mu + X$. $(a)$ Feynman diagram, $(b)$ in the laboratory frame.}
\label{feyn:nuNscattering}
\end{center}
\end{figure}

In the rest frame of the nucleon, which corresponds to the laboratory system (neglecting the Fermi motion) shown in Figure \ref{feyn:nuNscattering}(b), these momenta can be written as:
\begin{equation}
\begin{array}{lll}
k=(E,\mathbf{k}),&k^{\prime}=(E^{\prime},\mathbf{k}^{\prime}),&q=(\nu,\mathbf{q})\\
p_N=(M,\mathbf{0}),&p_X=(E_X,\mathbf{p}_X),&p_h=(E_h,\mathbf{p}_h)
\end{array}
\end{equation}
with M being the nucleon mass, $M=m_N$. Neglecting the mass of the $\mu$, the kinematic event variables can be expressed as follows:\footnote{The approximation ``$\simeq$'' indicates the neglected mass $m_\mu$, whereas ``$\approx$'' only holds for $E \gg M$}

\begin{itemize}

\item{The total energy in the center of mass system $\sqrt{s}$:
\begin{equation}
s = (k+p_N)^2 = 2ME+M^2 \approx 2ME
\end{equation}
}

\item{The negative square of the 4-momentum transfer $Q^2$:
\begin{equation}
Q^2 = -q^2 = -(k-k^{\prime})^2 = -(E-E^{\prime})^2+(\mathbf{k}-\mathbf{k}^{\prime}) \simeq 4EE^{\prime} \sin^2\frac{\theta}{2} > 0.
\end{equation}
where $\theta=\theta_{\mu}$ is the scattering angle of the muon.
}

\item{The energy transfer $\nu$ in the laboratory frame:
\begin{equation}
\nu = \frac{q \cdot p_N}{M} = E - E^{\prime} = E_X-M
\end{equation}
and
\begin{equation}
\nu_{\text{max}} \simeq \frac{2E^2}{2E+Mx_{\text{Bj}}} = E \text{  ~for  } x_{\text{Bj}}=0.
\end{equation}
with $x_{\text{Bj}}$ defined below in equation (\ref{eqn:x_bjorken}).
}

\item{The total energy $W$ of the outgoing hadrons $X$ in their center of mass frame corresponds to an effective mass of the hadronic final state:
\begin{equation}
W^2 = p_X^2 = E_X^2-\mathbf{p}_X^2 = (E-E^{\prime}+M)^2-(\mathbf{k}-\mathbf{k}^{\prime})^2= -Q^2+2M\nu+M^2
\label{eqn:wsqr}
\end{equation}
with
\begin{eqnarray}
W^2_{\text{max}} & \simeq & 2ME+M^2 = s\\
\text{where} & &\nu=\nu_{\text{max}} \simeq E \nonumber\\
 && Q^2 \simeq 0 \nonumber
\end{eqnarray}
}

\item{The Bjorken scaling variable $x_{\text{Bj}}$:\footnote{The boundaries for $x_{\text{Bj}}$ and $y$ are given, neglecting the mass $m_{\mu}$ of the outgoing muon.}
\begin{equation}
x_{\text{Bj}} = \frac{-q^2}{2q \cdot p_N} = \frac{Q^2}{2M\nu} \;\; \text{with:}\;\;  0\leq x_{\text{Bj}} \leq 1.
\label{eqn:x_bjorken}
\end{equation}

Combining equation (\ref{eqn:wsqr}) and (\ref{eqn:x_bjorken}) yields:
\begin{equation}
W^2 = M^2 + Q^2\left(\frac{1}{x_{\text{Bj}}}-1\right).
\end{equation}
}

\item{The inelasticity or relative energy transfer $y$:\footnotemark[\value{footnote}]
\begin{eqnarray}
y = \frac{q\cdot p_N}{k \cdot p_N} = \frac{\nu}{E} = 1 - \frac{E^{\prime}}{E} = \frac{Q^2}{2MEx_{\text{Bj}}}  \label{eqn:y_bjorken}\\
\text{with:}\;\; 0\leq y \leq \left(1+ \frac{Mx_{\text{Bj}}}{2E} \right)^{-1} \approx 1 \nonumber
\end{eqnarray}
From (\ref{eqn:x_bjorken}) and (\ref{eqn:y_bjorken}) another useful relation can be given:
\begin{equation}
yx_{\text{Bj}} = \frac{Q^2}{2ME} = \frac{Q^2}{s-M^2}
\end{equation}
}
\end{itemize}

For a given neutrino energy $E=E_{\nu}$, the measurement of two independent variables, e.q. $(E^{\prime},\theta)$ or $(Q^2,\nu)$ or $(x,Q^2)$ or $(x,y)$, is sufficient to characterize a scattering event of the form (\ref{eqn:nuNscattering}). 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Deep Inelastic Scattering}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
If a neutrino is scattered off a nucleon with sufficiently large $Q^2$, the nucleon will break apart. 
In the limit $Q^2 \gg M^2$, referred to as \emph{deep inelastic scattering} (DIS), this reaction can be described as scattering between a neutrino and a free quark with momentum $p_q = \xi p_N$ (see Figure \ref{feyn:DISscattering}). It can be shown that in lowest order perturbation theory $\xi = x_{\text{Bj}}$, i.\ e.\ the Bjorken scaling variable $x_{\text{Bj}}$ is equal to the fraction of the nucleon momentum that is carried by the interacting quark. The quark content of a nucleon is specified via the quark distribution or \emph{parton density functions}\footnote{The distribution functions $q(\xi)$ should not be confused with the Dirac spinors $f(x)$ introduced in Section \ref{sec:WeakInt}} $q(\xi)$ which are defined as follows:
\begin{equation}
\begin{array}{ccl}
q(\xi)d\xi & = & \text{Number of quarks q in the nucleon with}\\
& & \text{a momentum fraction between $\xi$ and $\xi+d\xi$.} 
\end{array}
\end{equation}
The distributions $u(\xi)$ and $d(\xi)$ can be divided into \emph{valence} quark and \emph{sea} quark distributions:
\begin{eqnarray}
u(\xi) & = & u_V(\xi) + u_S(\xi) \\  
d(\xi) & = & d_V(\xi) + d_S(\xi).
\end{eqnarray}
For symmetry reasons it is assumed that the following relations hold for the sea quark distributions:
\begin{equation} 
\begin{array}{ccccccc}
u_S(\xi) & = & \overline{u}(\xi) && s(\xi) & = &\overline{s}(\xi)\\
d_S(\xi) & = & \overline{d}(\xi) && c(\xi) & = &\overline{c}(\xi) 
\end{array}
\end{equation}
where the $\overline{q}(\xi)$ denote the anti-quark distributions. For a proton consisting of three valence quarks, two $u$ and one $d$, the distributions must fulfill:
\begin{eqnarray} 
\int_0^1 u_V(\xi) d\xi = \int_0^1 [u(\xi)-\overline{u}(\xi)] d\xi = 2 \\
\int_0^1 d_V(\xi) d\xi = \int_0^1 [d(\xi)-\overline{d}(\xi)] d\xi = 1.
\end{eqnarray}

\begin{figure}[!htpb]
\begin{center}
\fmfframe(5,10)(5,10){
\begin{fmfgraph*}(160,140)
\input{./Theory/FeynDiag/DISscattering.tex}
\end{fmfgraph*}
}
\caption[DIS neutrino-nucleon scattering]{Feynman diagram for DIS neutrino-nucleon scattering. The neutrino scatters off a quasi free quark $q_1$ causing the reaction $\nu q_1\rightarrow \mu q_2$. The amplitude for this process is proportional to the element, $U_{q_1q_2}$, of the CKM matrix.}
\label{feyn:DISscattering}
\end{center}
\end{figure}

In lowest order the differential cross section for deep inelastic neutrino-nucleon scattering can then be given as an incoherent sum of the differential cross sections for elastic neutrino-quark scattering:
\begin{equation}
\frac{d\sigma}{dx_{\text{Bj}}dy} = 
\sum_{q,q^{\prime}} q(x_{\text{Bj}})\frac{d\sigma}{dy}(\nu q \rightarrow \mu^- q^{\prime}) + 
\sum_{\overline{q},\overline{q}^{\prime}} \overline{q}(x_{\text{Bj}})\frac{d\sigma}{dy}(\nu \overline{q} \rightarrow \mu^- \overline{q}^{\prime}).
\label{eqn:discrosssection}
\end{equation}
The differential cross sections ${d\sigma}/{dy}$ correspond to scattering processes of elementary fermions and can easily be calculated. Neglecting the W-propagator for not too high energies (see Section \ref{section:FourFermionCS}: $sx_{\text{Bj}} \ll m_{W}^2$), they are given by 
\begin{equation}
\frac{d\sigma}{dy}(\nu q \rightarrow \mu^- q^{\prime}) = 
\frac{2 G_F^2}{\pi}x_{\text{Bj}}ME|U_{qq^{\prime}}|^2
\end{equation}
and
\begin{equation}
\frac{d\sigma}{dy}(\nu \overline{q} \rightarrow \mu^- \overline{q}^{\prime}) = 
\frac{2 G_F^2}{\pi}x_{\text{Bj}}ME|U_{qq^{\prime}}|^2(1-y)^2
\end{equation}
where $U_{qq^{\prime}}$ are the elements of the CKM matrix.
Taking advantage of $|U_{ud}|^2 + |U_{cd}|^2 \simeq |U_{us}|^2 + |U_{cs}|^2 \simeq 1$, the cross section (\ref{eqn:discrosssection}) becomes
\begin{equation}
\frac{d\sigma}{dx_{\text{Bj}}dy}(\nu N) = \sigma_0 \cdot 2x_{\text{Bj}} ( [d(x_{\text{Bj}})+s(x_{\text{Bj}})] + [\overline{u}(x_{\text{Bj}}) + \overline{c}(x_{\text{Bj}})](1-y)^2)
\end{equation}
for $W$ above the charm threshold ($W > \unit[2.5]{GeV/c^2}$), with
\begin{equation}
\sigma_0 = \frac{G_F^2ME}{\pi}= \unit[1.538\times 10^{-38}]{\frac{cm^2}{GeV}}\cdot E.
\end{equation}


An integration over $x_{\text{Bj}}$ and $y$ yields the total cross sections which are linear functions of the neutrino energy. As shown in Figure \ref{figure:neutrino_xsec}, this behavior is well confirmed by experiments.
\begin{figure}[!htpb]
\begin{center}
\includegraphics[width = 110mm]{./Theory/Figures/neutrino_xsec_2002}
\caption[Total charged current cross section]{${\sigma_\text{\text{cc}}}/{E_{\nu}}$ for the total charged current cross section of neutrino- and anti-neutrino-nucleon scattering, as a function of the neutrino energy. The original plot as well a the references of the individual measurements can be found in \cite{PDBook:2002}.}
\label{figure:neutrino_xsec}
\end{center}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Quasi Elastic Charm Production}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{section:theory:QEC}
In quasi elastic scattering events the neutrino interacts with the nucleon as a whole and leaves it intact. As in the case of elastic scattering, the reaction has only one degree of freedom because it involves two incoming and two outgoing particles with definite masses. Due to the mass difference between the initial and the final state baryon, as well as between the neutrino and the charged lepton, the charged current process is not completely elastic. The most prominent and well measured quasi elastic processes are
\begin{equation}
\begin{array}{ccc}
\nu_{\mu} + n  \rightarrow  \mu^- + p & & E_{\text{thr}}=\unit[110]{MeV}\\
\overline{\nu}_{\mu}  + p  \rightarrow  \mu^+ + n & & E_{\text{thr}}=\unit[113]{MeV}
\end{array}
\label{eqn:QEnp}
\end{equation}
where for neutrino energies above the threshold energy $E_{\text{thr}}$ a transition between the quarks of the first generation $u \leftrightarrow d$ is induced. As a consequence of the quark mixing, the same mechanism should be able to produce charmed baryons quasi elastically in the following reactions:
\begin{eqnarray}
\nu_{\mu} + n  & \rightarrow  & \mu^- + \lambdac(2285) \label{eqn:theory:qecneut1}\\
\nu_{\mu} + n  & \rightarrow  & \mu^- + \sigmacp(2455) \label{eqn:theory:qecneut2}\\
\nu_{\mu} + n  & \rightarrow  & \mu^- + \mathnormal{\Sigma}_c^{*+}(2520) \label{eqn:theory:qecneut3}
\end{eqnarray}
and
\begin{eqnarray}
\nu_{\mu} + p  & \rightarrow  & \mu^- + \sigmacpp(2455) \label{eqn:theory:qecprot1}\\
\nu_{\mu} + p  & \rightarrow  & \mu^- + \mathnormal{\Sigma}_c^{*++}(2530).
\label{eqn:theory:qecprot2}
\end{eqnarray}
In the processes (\ref{eqn:theory:qecneut1})-(\ref{eqn:theory:qecprot2}) a $d$ quark has to change into a $c$ quark. Hence, they are all \emph{Cabibbo suppressed}, i.\ e., they have a cross section proportional to $\sin^2\theta_c\simeq 0.05$.
Since for \emph{quasi elastic charm production} (QEC) the hadronic final state consists of only one charmed baryon, the threshold energy is lower than for DIS charm production where the hadronic final state must involve at least one baryon and one charmed meson. The lower bound for the energy of the hadronic system is thus given by:  
\begin{equation}
W_{\text{\tiny{QEC}}} > m_{\lambdac} = \unit[2285]{MeV / c^2}
\end{equation}
and
\begin{equation}
W_{\text{DIS}} > m_{p}+m_{D^0} = \unit[2802]{MeV / c^2}
\end{equation}
for QEC and DIS respectively. 
\begin{figure}[!htpb]
\begin{center}
\fmfframe(10,10)(10,10){
\begin{fmfgraph*}(120,100)
\input{./Theory/FeynDiag/QECscattering.tex}
\end{fmfgraph*}
}
\caption[Feynman diagram for quasi elastic charm production]{Feynman diagram for quasi elastic charm production.}
\label{feyn:QECscattering}
\end{center}
\end{figure}
The matrix element for the QEC process, shown in Figure \ref{feyn:QECscattering}, can be written as\footnote{Here, the $u_f(p)$ denotes the spinor of the particle $f$ in ``momentum-space''.}:
\begin{equation}
\mathcal{M} = \frac{G_F \sin\theta_C}{\sqrt{2}} 
\overline{u}_{\mu}(k^{\prime})\gamma_{\alpha}(1-\gamma_5)u_{\nu}(k)\langle B_c(p^{\prime)}|J^{\alpha}_{D^+}|N(p)\rangle 
\end{equation}
where $N$ and $B_c$ denote the initial and final state baryons, and the hadronic current $J^{\alpha}_{D^+}$ describes the quasi elastic transition.
In contrast to DIS, the hadronic current $J^{\alpha}_{D^+}$ is not calculable with perturbative QCD because the $q^2$ dependent, effective coupling constant of the strong interactions, $\alpha_s$, is of the order of one in this kinematic region.
However, if the effective interaction is assumed to be of the V-A type, the general form of the matrix element of the hadronic current \cite{LlewellynSmith:1971zm,Pais1971,Marshak:1969} is given by
\begin{equation}
\langle B_c(p^{\prime)}|J^{\alpha}_{D^+}|N(p)\rangle   =  \overline{u}_{B_c}(p^{\prime})\Gamma^{\alpha}u_N(p)
\end{equation}
and
\begin{equation}
\Gamma^{\alpha} =
\gamma^{\alpha}(g_V+g_A\gamma_5) +
\frac{i\sigma^{\alpha\beta}}{(m_N+m_{B_c})}q_{\beta}(f_V+f_A\gamma_5)+
iq^{\alpha}(h_V+h_A\gamma_5)
\label{eqn:theory:QECcurrent}
\end{equation}
with
\begin{equation}
\sigma^{\alpha\beta} = \frac{i}{2}(\gamma^{\alpha}\gamma^{\beta}-\gamma^{\beta}\gamma^{\alpha}).
\end{equation}
In general, the form factors $g_V$, $g_A$, $f_V$, $f_A$, $h_V$, $h_A$ are complex and depend on $q^2$. The invariance under \emph{time reversal} ($T$) implies, however, that all the form factors in (\ref{eqn:theory:QECcurrent}) are real. If \emph{charge symmetry} is assumed, the form factors $f_A$ and $h_V$, corresponding to the second class currents, have to be imaginary, hence 
\begin{equation}
f_A=h_V=0.
\end{equation}
In other words, there are no second class currents if both $T$ invariance and charge symmetry is assumed. The term corresponding to the form factor $h_A$ can be neglected, since it gives a contribution proportional to the muon mass. 
It can be shown that only three combinations of the six form factors can be determined if the helicities of the leptons are not measured \cite{LlewellynSmith:1971zm}. Neglecting the muon mass, the cross section can be written as:
\begin{equation}
\frac{d\sigma}{dQ^2} = \frac{G_F^2\sin^2{\theta_C}}{8\pi E^2}\left[-2q^2W_1+(4EE^{\prime}+q^2)W_2+\frac{E+E^{\prime}}{m_N}q^2W_3\right]
\label{eqn:theory:QECxsection}
\end{equation}
with structure functions
\begin{equation}
W_1 = \frac{1}{4m_N^2}\{[(m_{B_c}-m_N)^2-q^2](g_V+f_V)^2+[(m_{B_c}+m_N)^2-q^2]g_A^2 \},
\end{equation}
\begin{equation}
W_2 = g_V^2 - \frac{q^2}{(m_N+m_{B_c})^2}f_V^2+g_A^2
\end{equation}
and
\begin{equation}
W_3 = 2g_A(g_V+f_V)
\end{equation}
Since the center of mass energy of the hadronic final state $W$ is fixed to the mass of the charmed baryon, the reaction has only one degree of freedom. For a given neutrino energy a quasi elastic event can therefore be characterized by a single variable, e.\ g.\ $Q^2$. \nocite{Finjord:1975fz,Shrock:1975uk,Shrock:1976Err,Avilez:1976bb,Avilez:1976qi,Avilez:1978rt,Amer:1978ya,Kovalenko:1990zi}

\begin{table}[!htpb]
\begin{center}
\input{./Theory/Tables/QECpredictionSummary.tex}
\caption[Predicted quasi elastic charm cross sections]{Predicted QEC production cross sections for a neutrino energy of \unit[10]{GeV}. Also, the production cross section relative to the total charged current cross section is given.}
\label{table:theory:QECpredictionSummary}
\end{center}
\end{table}% \cite{Mangano:2001mj}

Many authors have given predictions for the cross sections of QEC, based on the formula (\ref{eqn:theory:QECxsection}). An overview of the various results is given in Table \ref{table:theory:QECpredictionSummary}, where the cross section values are given for a neutrino energy of \unit[10]{GeV}. A common feature of all the models is a nearly constant cross section for neutrino energies above \unit[15]{GeV}. The differences between the predictions, which can be more than one order of magnitude, arise from the fact that the form factors cannot be established on the basis of the theory. In the calculations \cite{Finjord:1975fz,Shrock:1975uk,Shrock:1976Err,Avilez:1976bb,Avilez:1976qi,Avilez:1978rt,Amer:1978ya} the $q^2$ dependence of the form factors is parametrized with dipole formulas
\begin{eqnarray}
D(q^2) &\propto& \frac{1}{(1-\frac{q^2}{m_{ex}^2})^2}\;\;\;\text{(dipole)}\\
m_{ex} &=& \text{mass of the virtual exchange meson} \nonumber
\end{eqnarray}
which are the empirical result of the analysis of experimental data on the electromagnetic and weak nucleon form factors.


In this thesis the calculations of Kovalenko \cite{Kovalenko:1990zi} and those of Shrock and Lee \cite{Shrock:1975uk,Shrock:1976Err} are used. The model of Kovalenko tries to give an upper limit for the QEC cross section by taking advantage of the \emph{local duality} \cite{Bloom:1971ye}, which establishes a relation between the structure function $F^{th}(x,Q^2)$ of DIS, calculated in QCD, and the observed structure function $F^{ph}(x,Q^2)$, which at small $Q^2$ contains resonance peaks corresponding to the ground and excited states of baryons. The average of the two structure functions coincides to good accuracy, both, over the whole range of variation $0\leq x\leq 1$ (global duality)
\begin{equation}
\int_0^1[F^{th}(x,Q^2)-F^{ph}(x,Q^2)]dx\simeq 0,
\end{equation}
as well as in the vicinity of an individual resonance $x_{\text{min}}\leq x\leq x_{\text{max}}$ (local duality)
\begin{equation}
\int_{x_{\text{min}}}^{x_{\text{max}}}[F^{th}(x,Q^2)-F^{ph}(x,Q^2)]dx\simeq 0.
\label{eqn:localDuality}
\end{equation}
A modified version of these relations, taking into account some of the dominant corrections of $F^{th}(x,Q^2)$ in the region of small and moderate $Q^2$, can be used for an estimation of the structure functions $W_1$, $W_2$ and $W_3$.

The choice of the calculations of Shrock and Lee as a reference model is somewhat arbitrary in the sense that there are no fundamental formal discrepancies compared to the models \cite{Finjord:1975fz,Avilez:1976bb,Avilez:1976qi,Avilez:1978rt,Amer:1978ya}. Using the approximate $SU(4)$ symmetry of the strong interaction\footnote{If the masses of the quarks $u$,$d$,$c$,$s$ are assumed to be equal, the strong interaction becomes invariant under $SU(4)$ ``rotations'' of these quark flavors}, the form factors in the model of Shrock and Lee are derived from those found in the reactions (\ref{eqn:QEnp}) and the neutron decay. 
The form factors are combinations of dipole terms with parameters $m_{ex}$ being set to the masses of the exchanged charmed mesons. A more detailed description of the two models will be given in Section \ref{section:simulation:QEC}.


==> abstract.tex <==
%\chapter{Abstract}
%\vspace{-1cm}
\typeout{}
%\markboth{ABSTRACT/ZUSAMMENFASSUNG}{ABSTRACT/ZUSAMMENFASSUNG}
\addcontentsline{toc}{chapter}{\numberline{}Abstract}

\mbox{}
\vspace{0.5cm}
\mbox{}

\noindent
\begin{center}
{\Large \bf Abstract}
\end{center}

\noindent
A first study of the stopping muons measured with the very large
liquid argon (LAr) time projection chamber, ICARUS T600, is
presented. The ICARUS detector will be installed in the Gran Sasso
underground laboratory in Italy, to study neutrino oscillations and to
search for nucleon decays. The studied muons have been produced by
interactions of cosmic rays in the atmosphere and stopped inside the
detector's sensitive volume. The data have been acquired during the
technical run, testing the detector at the surface of the earth in
Pavia (Italy) during summer 2001. We have performed a first analysis
of 259 stopping muon events from three days of data taking. The tools
for the three-dimensional reconstruction of general events have been
developed and optimized for the stopping muon event topology. The
events reconstructed with these tools have been used to perform
several analyses. First, we have determined the attachment rate of the
drift electrons to electro-negative impurities in the LAr volume,
parameterized by the free electron lifetime. The measured lifetimes
for the considered data taking period are between 1.2 and 1.4~ms. For
an electric drift field of 500 V/cm, this translates into a mean drift
distance of electrons, before being captured by impurities, of 1.9 to
2.2~m, which has to be compared to the longest possible drift distance
in the detector of 1.5~m. The charge collected at the wires of the
drift chamber has been corrected for the effect of electron attachment
in order to calculate the charge of drift electrons per crossed
distance produced by the ionizing particle (muon) along its track. A
comparison of the corrected measured charge with the theoretical
expectation from the energy loss has been used to perform a
determination of the electron recombination factor ($R$) as a function
of the energy loss in LAr, at an electric field of 500~V/cm. A linear
dependence of $R^{-1}$ on $dE/dx$ has been found, with a slope of 0.13
$\pm$ 0.01~cm/MeV and a value of $R_{mip}=0.604 \pm 0.008$ for minimum
ionizing particles. These results are used for a complete calorimetric
reconstruction of the event sample. Next, we have studied the sample
of muon decay electrons. We have measured the value of the Michel
parameter $\rho$ from the electron energy spectrum, obtaining $\rho =
0.77\pm 0.22
\textrm{ (stat.)} \pm 0.10 \textrm{ (syst.)}$. A reduction of the
error to an overall $10\%$ is expected when the whole event sample
available from the T600 technical run will be included. From a
comparison of the measured and the a Monte Carlo generated electron
energy spectra, the energy resolution in the range [0--53]~MeV has
been determined to be $\sigma/E = (9\pm 1)\%/\sqrt{E[\textrm{MeV}]}
\oplus (3.9\pm 0.2)\%$. Finally, we have studied the energy resolution
which can be achieved when the electron energy is computed from the
track length; the resolution found is about 15$\%$ for electron
energies above 30~MeV, increasing to about 35$\%$ at 10~MeV.

These results demonstrate the capability of the novel liquid argon
experimental technique to produce high quality data to perform
physics analyses, in particular the study of neutrino oscillations
with the data collected in the Gran Sasso Laboratory, starting in
2003.

A detailed description of the Slow Control system of the ICARUS
T600 detector, and of the off-line analysis of the data acquired
during the technical run, is also presented. This system was
intended to monitor the behaviour of the detector during the
different phases of the run. From the results some important
conclusions could be drawn, which lead to a better understanding
of the thermodynamical and mechanical behaviour of the detector as
a large cryogenic device, using ultra-pure LAr.


